Linking Threat Tactics, Techniques, and Patterns with Defensive Weaknesses, Vulnerabilities and Affected Platform Configurations for Cyber Hunting

Many public sources of cyber threat and vulnerability information exist to help defend cyber systems. This paper links MITRE's ATT&CK MATRIX of Tactics and Techniques, NIST's Common Weakness Enumerations (CWE), Common Vulnerabilities and Exposures (CVE), and Common Attack Pattern Enumeration and Classification list (CAPEC), to gain further insight from alerts, threats and vulnerabilities. We preserve all entries and relations of the sources, while enabling bi-directional, relational path tracing within an aggregate data graph called BRON. In one example, we use BRON to enhance the information derived from a list of the top 10 most frequently exploited CVEs. We identify attack patterns, tactics, and techniques that exploit these CVEs and also uncover a disparity in how much linked information exists for each of these CVEs. This prompts us to further inventory BRON's collection of sources to provide a view of the extent and range of the coverage and blind spots of public data sources.

==> figures/bron_network_schematic.tex <==
\begin{tikzpicture}[
cve/.style={circle, draw=cyan, very thick, minimum size = 7mm},
cpe/.style={circle, draw=violet, very thick, minimum size = 7mm},
network-nodes/.style={circle, draw=orange, very thick, minimum size = 7mm},
]
%cve nodes
\node[minimum size = 10 mm] (cve-type) at (0,-7.0) {CVE};
\node[cve] (cve1) at (3.4,-7) {};
\node[cve] (cve2) at (4.8,-7) {};
\node[cve] (cve3) at (6.2,-7) {};
\node[cve] (cve4) at (7.6,-7) {};
\node[cve] (cve5) at (9.0,-7) {};

%cpe nodes
\node[minimum size = 10 mm] (cpe-type) at (0,-8.5) {CPE};
\node[cpe] (cpe1) at (3,-8.5) {};
\node[cpe] (cpe2) at (4.2,-8.5) {};
\node[cpe] (cpe3) at (5.4, -8.5) {};
\node[cpe] (cpe4) at (6.6,-8.5) {};
\node[cpe] (cpe5) at (7.8,-8.5) {};
\node[cpe] (cpe6) at (9.0,-8.5) {};

%cve-cpe arrows
\draw[<->,very thick] (cve1) -- (cpe1);
\draw[<->, very thick] (cve2) -- (cpe1);
\draw[<->,very thick] (cve2) -- (cpe2);
\draw[<->, very thick] (cve3) -- (cpe2);
\draw[<->, very thick] (cve4) -- (cpe2);
\draw[<->, very thick]  (cve3) -- (cpe3);
\draw[<->, very thick]  (cve4) -- (cpe3);
\draw[<->, very thick] (cve5) -- (cpe4);
\draw[<->, very thick] (cve4) -- (cpe5);
\draw[<->, very thick] (cve4) -- (cpe6);
\draw[<->, very thick] (cve5) -- (cpe5);

%network nodes
\node[minimum size = 10 mm] (network-type) at (0,-9.5) {Network Nodes};
\node[network-nodes] (node1) at (4, -9.5) {};
\node[network-nodes] (node2) at (5.5, -9.5) {};
\node[network-nodes] (node3) at (7, -9.5) {};
\node[network-nodes] (node4) at (8.5, -9.5) {};
\node[network-nodes] (node5) at (10, -9.5) {};

%cpe-network arrows
\draw[black, thick] (3,-9) rectangle (10.5, -9.9);
\draw[dashed] (cpe1) -- (node1);
\draw[dashed] (cpe2) -- (node1);
\draw[dashed] (cpe3) -- (node2);
\draw[dashed] (cpe3) -- (node3);
\draw[dashed] (cpe4) -- (node5);
\draw[dashed] (cpe5) -- (node4);
\end{tikzpicture}





==> figures/medical_cve_contents.tex <==
\begin{tikzpicture}[
tactic/.style={circle, draw=green, very thick, minimum size = sqrt(4)+7 mm, inner sep = 2pt},
techniq2/.style={circle, draw=red, very thick, minimum size = sqrt(22)+7 mm, inner sep = 2pt},
capec2/.style={circle, draw=blue, very thick, minimum size = sqrt(22)+7 mm, inner sep = 2pt},
capec3/.style={circle, draw=blue, very thick, minimum size = sqrt(52)+7 mm, inner sep = 2pt},
cwe2/.style={circle, draw=magenta, very thick, minimum size = sqrt(2)+7 mm, inner sep = 2pt},
cwe3/.style={circle, draw=magenta, very thick, minimum size = sqrt(2)+7 mm, inner sep = 2pt},
cve1/.style={circle, draw=cyan, very thick, minimum size = sqrt(3)+7 mm, inner sep = 2pt},
cve2/.style={circle, draw=cyan, very thick, minimum size = sqrt(2)+7 mm, inner sep = 2pt},
cpe2/.style={circle, draw=violet, very thick, minimum size = sqrt(5)+7 mm, inner sep = 2pt},
]

%Tactic row
%\node[minimum size = 10mm] (floating-type) at (2, 0) {Neither Above and Below};
%\node[minimum size = 10mm] (previous-connection) at (6,0) {Only Layer Above};
%\node[minimum size = 10 mm] (both-connection) at (10,0) { Both Above and Below};
%\node[minimum size = 10mm] (next-connection) at (14,0) { Only Layer Below};

\node[minimum size = 20 mm] (tactic-type) at (0,-1) {TACTIC}; 
\node[tactic] (tactic1) at (4,-1) {5};

%Technique row
\node[minimum size = 20 mm] (technique-type) at (0,-3) {TECHNIQ}; 

\node[techniq2] (techniq2) at (4,-3) {25};


\draw (tactic1) -- (techniq2);


%capec
\node[minimum size = 20 mm] (capec-type) at (0,-5) {CAPEC}; 
\node[capec2] (capec2) at (2,-5) {22};
\node[capec3] (capec3) at (4, -5) {52};

\draw (techniq2) -- (capec2);


%cwe
\node[minimum size = 20 mm] (cwe-type) at (0,-7) {CWE}; 

\node[cwe2] (cwe2) at (2, -7) {2};
\node[cwe3] (cwe3) at (4, -7) {2};

\draw (capec3) -- (cwe2); 
\draw(capec2) -- (cwe2);


%cve
\node[minimum size = 20 mm] (cve-type) at (0,-9) {CVE};
\node[cve1] (cve1) at (2, -9) {3};
\node[cve2] (cve2) at (4, -9) {6};

\draw (cwe3) -- (cve2);
\draw (cwe2) -- (cve2);

%cpe
\node[minimum size = 20 mm] (cpe-type) at (0, -11) {\platform};
\node[cpe2] (cpe1) at (3, -11) {5};


\draw (cve2) -- (cpe1);

\end{tikzpicture}

%




==> figures/trends_gaps.tex <==
\subsection{Gap and Trend Analysis}\label{sec:GapTrendAnalysis}

Are there gaps within \bron and have they been shifting over time?

The general trend in the number of \VULNERABILITY paths increases as more \VULNERABILITIES are recorded.
In 2008, there we can observe a spike in the number of \VULNERABILITY paths compared to 2007 and 2009.
For example, there are 620, 1527 and 816 paths respectively originating at \TACTICS in 2007, 2008 and 2009.
Paths originating at  \ATTACKPATTERN{s} trend from 2,251 in 2007, 5,369 in 2008 to  3,141 in 2009.
We hypothesize this spike may be due to more records of \VULNERABILITIES in  linked to \ATTACKPATTERN{s} in 2008.

Longer term, the number of connected \VULNERABILITIES compared to the total number of reported \VULNERABILITIES increases over the years, with most of the growth occurring after 2006. The percentage of reported \VULNERABILITIES with paths from \TACTICS increased from 2.16\% in 1999 to 17.00\% in 2020, while the percentage of \VULNERABILITIES that are not connected to \WEAKNESS{es} decreased from 95.87\% in 1999 to 28.32\% in 2020 as seen in Figure~\ref{fig:cve_connect_to_data_types_pct}. These changes show substantial information growth as more reported \VULNERABILITIES are linked to \TACTICS, \TECHNIQS, \ATTACKPATTERN{s}, and \WEAKNESS{es} than earlier.

There are also more \ATTACKPATTERN paths to \VULNERABILITIES than other types of \VULNERABILITY paths for many of the years.
This suggests that some \VULNERABILITIES are linked to \WEAKNESS{es} and \ATTACKPATTERN{s} but not related to a \TECHNIQ.
This observation is reasonable given that only 10\% of \ATTACKPATTERN{s} are connected to both \TECHNIQ entries and \WEAKNESS{es}, as we have already observed. While the quantity of paths has increased between 1999 and 2020, it is hindered by the lack of connections from many \ATTACKPATTERN{s} to \TECHNIQS.


